Phase transitions in D-dimensional Gauss-Bonnet-Born-Infeld AdS black holes

In this paper, we have investigated the phase transition in black holes when Gauss-Bonnet corrections to the spacetime curvature and Born-Infeld extension in stress-energy tensor of electromagnetic field are considered in a negative cosmological constant background. It is evident that the black hole undergoes a phase transition as the specific heat capacity at constant potential shows discontinuities. Further, the computation of the free energy of the black hole, the Ehrenfest scheme and the Ruppeiner state space geometry analysis are carried out to establish the second order nature of this phase transition. The effect of non-linearity arising from Born-Infeld electrodynamics is also evident from our analysis. Our investigations are done in general D-spacetime dimensions with D > 4, and specific computations have been carried out in D = 5, 6, 7 spacetime dimensions.

==> Response_TEX 1/umbclogo-2003-01.tex <==
% UMBC logo
%
% This file is \included in PPRumbc*.sty
%
% Rouben Rostamian
% September 2002

\definecolor{shadowcolorA}{gray}{0.7}
\definecolor{shadowcolorB}{gray}{0.2}
\newcommand{\umbclogo}{%
	{\fontfamily{phv}\fontseries{b}\fontshape{sl}\fontsize{7}{7}%
	\selectfont%
	\makebox[0pt][l]{\raisebox{-0.20ex}[0pt][0pt]{\color{shadowcolorA}\hspace*{.20ex}UMBC}}%
	\makebox[0pt][l]{\raisebox{-0.10ex}[0pt][0pt]{\color{shadowcolorB}\hspace*{.10ex}UMBC}}%
	{\red UMBC}\hspace{.20ex}%
}}

% Define custumized bullets if the tribullet.sty package is available.
\IfFileExists{tribullet.sty}{
	\RequirePackage{tribullet}
	\myitem{1}{\raisebox{0.60ex}{\tribullet[1.40ex]{red}}}
	\myitem{2}{\raisebox{0.55ex}{\tribullet[1.30ex]{blue}}}
	\myitem{3}{\raisebox{0.50ex}{\tribullet[1.25ex]{cyan}}}
}{}


==> umbclogo-2003-01.tex <==
% UMBC logo
%
% This file is \included in PPRumbc*.sty
%
% Rouben Rostamian
% September 2002

\definecolor{shadowcolorA}{gray}{0.7}
\definecolor{shadowcolorB}{gray}{0.2}
\newcommand{\umbclogo}{%
	{\fontfamily{phv}\fontseries{b}\fontshape{sl}\fontsize{7}{7}%
	\selectfont%
	\makebox[0pt][l]{\raisebox{-0.20ex}[0pt][0pt]{\color{shadowcolorA}\hspace*{.20ex}UMBC}}%
	\makebox[0pt][l]{\raisebox{-0.10ex}[0pt][0pt]{\color{shadowcolorB}\hspace*{.10ex}UMBC}}%
	{\red UMBC}\hspace{.20ex}%
}}

% Define custumized bullets if the tribullet.sty package is available.
\IfFileExists{tribullet.sty}{
	\RequirePackage{tribullet}
	\myitem{1}{\raisebox{0.60ex}{\tribullet[1.40ex]{red}}}
	\myitem{2}{\raisebox{0.55ex}{\tribullet[1.30ex]{blue}}}
	\myitem{3}{\raisebox{0.50ex}{\tribullet[1.25ex]{cyan}}}
}{}

